Design and Validation of a Multi-Arm Relocatable Manipulator for Space Applications

This work presents the computational design and validation of the Multi-Arm Relocatable Manipulator (MARM), a three-limb robot for space applications, with particular reference to the MIRROR (i.e., the Multi-arm Installation Robot for Readying ORUs and Reflectors) use-case scenario as proposed by the European Space Agency. A holistic computational design and validation pipeline is proposed, with the aim of comparing different limb designs, as well as ensuring that valid limb candidates enable MARM to perform the complex loco-manipulation tasks required. Motivated by the task complexity in terms of kinematic reachability, (self)-collision avoidance, contact wrench limits, and motor torque limits affecting Earth experiments, this work leverages on multiple state-of-art planning and control approaches to aid the robot design and validation. These include sampling-based planning on manifolds, non-linear trajectory optimization, and quadratic programs for inverse dynamics computations with constraints. Finally, we present the attained MARM design and conduct preliminary tests for hardware validation through a set of lab experiments.

==> appendices.tex <==
\appendices
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Friction Cones Rotation Matrix}\label{appendix:RotM}
The matrix \mbox{$\bm R_\mathcal{S} \in \mathbb R^{3 \times 3}$} maps the contact forces in a local reference frame.
One can choose \mbox{$\bm R_\mathcal{S}$} such that the $z$-axis represents the normal component of the contact force, thus satisfying \mbox{$\bm R_\mathcal{S} \ \bm n_\mathcal{S} = \begin{bmatrix} 0 & 0 & 1 \end{bmatrix}^T$}, e.g. as follows:
\begin{equation}\label{eq:rotation_matrix}
    \bm R_\mathcal{S} = 
    \begin{bmatrix}
    \frac{n_{\mathcal{S}_y}}{\sqrt{n_{\mathcal{S}_x}^2 + n_{\mathcal{S}_y}^2}} & -\frac{n_{\mathcal{S}_x}}{\sqrt{n_{\mathcal{S}_x}^2 + n_{\mathcal{S}_y}^2}} & 0\\
    \frac{n_{\mathcal{S}_x} n_{\mathcal{S}_z}}{\sqrt{n_{\mathcal{S}_x}^2 + n_{\mathcal{S}_y}^2}} & \frac{n_{\mathcal{S}_y} n_{\mathcal{S}_z}}{\sqrt{n_{\mathcal{S}_x}^2 + n_{\mathcal{S}_y}^2}} & -\sqrt{n_{\mathcal{S}_x}^2 + n_{\mathcal{S}_y}^2}\\
    n_{\mathcal{S}_x} & n_{\mathcal{S}_y} & n_{\mathcal{S}_z}
    \end{bmatrix}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Simplified Dynamic Models}\label{appendix:reduced_models}
% \subsection{Reduced Model with Mass-Less Rope}\label{appendix:reduced_model_massless_rope} 
% We can consider a reduced version of the model presented in SubSec.~\ref{subsec:complete_model}, in particular we here consider a mass-less rope. By denoting with $n = 6$ and $n_u = 7$ the number of actuated and unactuated degrees-of-freedom (DoFs), respectively, the joint variables can be now collected in the vector \mbox{$\bm{q}\in \mathbb{R}^{n+n_u}$}, as follows:
% \begin{equation} 
%     \bm{q} = 
%     \begin{bmatrix}
%         \bm{p}_{\text{fb}}^T &
%         \boldsymbol{\rho}_{\text{fb}}^T & 
%         \bm{q}_{\text{ll}}^T &
%         \bm{q}_{\text{lr}}^T
%     \end{bmatrix}^T
%     \label{eq:free_joint_state}
% \end{equation}
% notice that w.r.t. the model described in~\eqref{eq:joint_state}, we here discard the three joints located at the \emph{master-point}. Consequently the generalized coordinates velocities \mbox{$\bm{\nu}\in \mathbb{R}^{n+n_u-1}$} and accelerations \mbox{$\bm{\dot{\nu}}\in \mathbb{R}^{n+n_u-1}$} are given by:
% \begin{subequations}
% \begin{align}
%     & \begin{matrix}
%         \bm{\nu} = 
%         \begin{bmatrix}
%             \bm{\dot{p}}_{\text{fb}}^T &
%             \boldsymbol{\omega}_{\text{fb}}^T & 
%             \bm{\dot{q}}_{\text{ll}}^T & 
%             \bm{\dot{q}}_{\text{lr}}^T 
%         \end{bmatrix}^T
%          \end{matrix} \\
%   & \begin{matrix}
%         \bm{\dot{\nu}} = 
%         \begin{bmatrix}
%             \bm{\ddot{p}}_{\text{fb}}^T & 
%             \boldsymbol{\dot{\omega}}_{\text{fb}}^T & 
%             \bm{\ddot{q}}_{\text{ll}}^T &
%             \bm{\ddot{q}}_{\text{lr}}^T 
%         \end{bmatrix}^T
%     \end{matrix}
% \end{align}
% \end{subequations}

% In this work, a rope is connected to the robot at the \textit{master-point} $\bm{p}_{\text{b}}$, i.e. a point fixed to the robot main body from the \textit{anchor-point} $\bm{p}_{\text{r}}$. 
% The \textit{anchor-point} is assumed to be fixed w.r.t. the world reference frame as shown in \eqref{eq:anchor_point_constraint}. 
% The effect of the rope on the robot dynamics is to impose a scalar, \emph{holonomic constraint} on it, of the mathematical form $h_{\text{rope}}(\bm{q}) = 0$, where $h_{\text{rope}}: \mathbb{R}^n \rightarrow \mathbb{R}$ has the following expression:
% \begin{equation}
%     \label{eq:rope_constraint}
%     h_{\text{rope}}(\bm{q}) = \tfrac{1}{2}\lVert \bm{p}_{\text{b}}(\bm q) - \bm{p}_{\text{r}} \rVert^2_2 - \tfrac{1}{2} \ell_r^2,
% \end{equation}
% where the rope length $\ell_r$ is considered to be possibly time-varying.
%  Differentiation of \eqref{eq:rope_constraint} yields 
% \begin{equation}
% \begin{aligned}
% \bm{J}_{\text{rope}}\bm{\nu} &= \ell_r\dot{\ell}_r  \\
% \bm{J}_{\text{rope}}\bm{\dot{\nu}} + \bm{\dot{J}}_{\text{rope}}\bm{\nu} &= \ell_r\ddot{\ell}_r + \dot{\ell}^2_r
% \end{aligned} ,
% \end{equation}
% where the rope constraint Jacobian $\bm{J}_{\text{rope}}$ is given by
% \begin{equation}
%   \bm{J}_{\text{rope}} = \left( \bm{p}_{\text{b}}(\bm{q}) - \bm{p}_{\text{r}} \right)^T \bm{J}_\text{b},
% \end{equation}
% and its rate of change $\bm{\dot{J}}_{\text{rope}}$ can be obtained as
% \begin{equation}
% \begin{aligned}
% \bm{\dot{J}}_{\text{rope}} &= \bm{\dot{p}}_{\text{b}}(\bm{q}, \bm{\nu})^T\bm{J}_\text{b} + \left( \bm{p}_{\text{b}}(\bm{q}) - \bm{p}_{\text{r}} \right)^T\bm{\dot{J}}_\text{b} \\
% &= \bm{\nu}^T\bm{J}_\text{b}^T\bm{J}_\text{b} + \left( \bm{p}_{\text{b}}(\bm{q}) - \bm{p}_{\text{r}} \right)^T\bm{\dot{J}}_\text{b} 
% \end{aligned}.
% \end{equation}
% To enforce the constraint \eqref{eq:rope_constraint}, a scalar generalized force \mbox{$f_r\in\mathbb{R}$} must act on the robot free dynamics, leading to the following \textit{rope-constrained dynamics}
% \begin{equation}
%     \begin{cases}
%     \bm{B}\bm{\dot{\nu}} + \bm{h} &= \bm{S}\bm{\tau} + \bm{J}_\text{C}^T\bm{F}_\text{C} + \bm{J}_{\text{rope}}^Tf_r \\ 
%     \bm{J}_{\text{rope}}\bm{\dot{\nu}} + \bm{\dot{J}}_{\text{rope}}\bm{\nu} &= \ell_r\ddot{\ell}_r + \dot{\ell}^2_r
%     \\f_r \leq 0
%     \end{cases}
%     \label{eq:reduced_model_rope_constrained_dynamics}
% \end{equation}
% where here the selection matrix $\bm{S}$ has the form:
% \begin{equation}
%     \label{eq:reduced_model_matrixS}
%     \bm{S} = \begin{bmatrix} 
%                 \bm{0}_{6\times n} & 
%                 \bm{I}_{6\times n} 
%              \end{bmatrix}^T.
% \end{equation}

% In order to get more physical insight on the generalize force $f_r$, its action on the joint dynamics $\bm{\tau}_r = \bm{J}_{\text{rope}}^Tf_r$ can be rewritten as follows:
% \begin{equation} \label{eq:tau_r}
% \begin{aligned}
%     \bm{\tau}_r = \bm{J}_{\text{rope}}^T f_r = \bm{J}_\text{b}^T\underbrace{\left( \bm{p}_{\text{b}}(\bm{q}) - \bm{p}_{\text{r}} \right)\,f_r}_{= \bm{F}_r}.
% \end{aligned}
% \end{equation}
% As expected, according to~\eqref{eq:tau_r} the action of the rope constraint~\eqref{eq:rope_constraint} is a pure force $\bm{F}_r = \left( \bm{p}_{\text{b}}(\bm{q}) - \bm{p}_{\text{r}} \right)\,f_r$, in the direction of the rope. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Rope-Assisted Robot Centroidal Dynamics}\label{appendix:centroidal_dynamics}
% By expressing the rate of change of the total linear and angular momentum of the system in a frame anchored at the Center of Mass (CoM), that has origin $\bm p_{\text{CoM}} \in \mathbb R^3$ and orientation of the inertial frame, 
% %see \cite{orin2013centroidal,saccon2017centroidal}, 
% see \cite{orin2013centroidal}, 
% called \textit{centroidal momentum}, the dynamics expressed in \eqref{eq:floatingdyn_unact} can be rewritten as:
% \begin{equation}
%     \label{eq:centroidal_dyn} 
%     \bm{A}(\bm{q})\bm{\dot{\nu}} + \bm{\dot{A}}(\bm{q},\bm{\nu}) \bm{\nu} = m \bm g + {\bm{G}_{\text{CD}}} 
%     \left[
%     \begin{array}{c} 
%     \bm{F}_\text{C} \\ 
%     \hdashline[2pt/2pt] 
%     \bm{F}_\text{r} 
%     \end{array}
%     \right]
% \end{equation}
% This formulation is called \textit{centroidal dynamics} (CD) \cite{orin2013centroidal}, where $\bm{A}(\bm{q}) \in\mathbb{R}^{6 \times (n+n_u-1)}$ is denoted as \textit{centroidal momentum matrix} (CMM), which maps the velocities, and therefore momentum, of each individual body into the common reference frame at the CoM. The gravitazional twist is given by \mbox{$\bm g \in\mathbb{R}^{6}$}, while \mbox{$m \in\mathbb{R}$} is the mass of the entire robot. 
% The left-hand side of \eqref{eq:centroidal_dyn} denotes the rate of change of the centroidal momentum, i.e.: 
% \begin{equation}
% \frac{d}{dt}(\bm{A}\bm{\nu}) =  \begin{bmatrix} \bm{F}\\ \bm{\dot{L}} \end{bmatrix}
% \end{equation}
% which for all mechanical systems must equal the net external wrench on the system  (right-hand side).
% Finally, the centroidal dynamics grasp matrix $\bm{G}_{\text{CD}}\in\mathbb{R}^{6\times k}$ is given by:
% \begin{equation}
%     \label{eq:grasp-structure_centroidal}
%     \bm{G}_{\text{CD}} = \begin{bmatrix} \bm{I}_3 &  \bm{I}_3 & \bm{I}_3  \\
%                          \bm{S}_\times(\bm{p}_{\text{CoM}} - \bm{p}_{\text{Cl}}) 
%                          &  \bm{S}_\times(\bm{p}_{\text{CoM}} - \bm{p}_{\text{Cr}}) 
%                          & \bm{S}_\times(\bm{p}_{\text{CoM}} - \bm{p}_{\text{b}}) 
%                          \end{bmatrix}
% \end{equation}
% \par
% The model in \eqref{eq:centroidal_dyn} is subject to the same constraints previously introduced in Sec. \ref{subsec:complete_model} except for \eqref{eq:torque_rope_unilaterality}, i.e. the \textit{rope pulling constraint}, since the dependency on $\bm \tau$ is now missing. 
% To this end, let $\bm n_\text{r} \in \mathbb{R}^3$ be the rope unit vector:
% \begin{equation}\label{eq:rope_force_equality}
%     \bm n_\text{r} = 
%     \frac{\bm{p}_{\text{b}}-\bm{p}_{\text{r}}}{\Arrowvert\bm{p}_{\text{b}}-\bm{p}_{\text{r}}\Arrowvert_2}.
% %    \approx 
% %    \frac{\bm{p}_{\text{CoM}}-\bm{p}_{\text{r}}}{\Arrowvert\bm{p}_{\text{CoM}}-\bm{p}_{\text{r}}\Arrowvert_2}
% \end{equation}
% % being \mbox{$\bm{p}_{\text{b}} \in \mathbb{R}^3$} the position of the master-point.
% Consequently, the rope pulling effect can be formulated as an equality constraint, expressed w.r.t. the rope force $\bm{F}_{\text{r}}$, i.e.:
% \begin{equation}
% \bm{F}_\text{r} \cdot \bm n_\text{r} = -\Arrowvert \bm{F}_\text{r} \Arrowvert_2 
% \label{eq:centroidal_dynamics_rope_constraint}
% \end{equation}
% \begin{equation}
%     \left(\bm{I}_{3\times 3} - \bm{n}_\text{r}\bm{n}_\text{r}^T\right)\,\bm{F}_\text{r} = \bm{0}
% \end{equation}
% enforcing that a pure pulling action is exerted along $\bm n_\text{r}$.\\
% %%%
% Notice that~\eqref{eq:centroidal_dynamics_rope_constraint} can be alternatively written as:
% %%% 
% \begin{equation}\label{eq:rope_force_inequality}
% \mathcal F(\bm{F}_{\text{r}}, \bm n_\text{r}):=
% \begin{cases}
% \bm{F}_\text{r} \cdot \bm n_\text{r}  < 0\\
% \Arrowvert \bm{F}_\text{r}^t \Arrowvert_2  =  0
% \end{cases}
% \end{equation}
% %%%
% A linear version of \eqref{eq:rope_force_inequality} can be obtained by choosing a rotation matrix \mbox{$\bm R_\text{r}$} as in \eqref{eq:rotation_matrix}, that maps $\bm{F}_{\text{r}}$ in a local reference frame 
% % at the \textcolor{red}{(master-point?)} anchor-point 
% such that \mbox{$\bm R_\text{r} \ \bm n_\text{r} = \begin{bmatrix} 0 & 0 & 1 \end{bmatrix}^T$}, yielding: 
% \begin{equation}
% \bm{b}_\text{r,l} \leq \bm{R}_\text{r}\,\bm{F}_\text{r} \leq \bm{b}_\text{r,u}
% \end{equation}
% with $\bm{b}_\text{r,l}=\begin{bmatrix} 0 & 0 & -\infty \end{bmatrix}^T$ and $\bm{b}_\text{r,u}=\begin{bmatrix} 0 & 0 & 0 \end{bmatrix}^T$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Integration Methods}\label{appendix:integration}
% % http://web.mit.edu/10.001/Web/Course_Notes/Differential_Equations_Notes/node5.html
% % http://www.cmth.ph.ic.ac.uk/people/a.mackinnon/Lectures/compphys/node11.html
% Any ODE in $n$ unknowns can be written in the general first-order form:
% \begin{equation}
%     \dot{\bm{x}} = \bm f(\bm x, \bm u) 
% \end{equation}
% where $\bm{x}$ and $\bm f$ are $n$-component vectors.

% \subsection{Euler Method}
% The forward Euler method (FE) computes $\bm{x}_{k+1}$ as:
% \begin{equation}
%     \bm{x}_{k+1}=\bm{x}_k + dt \bm{f}(\bm{x}_k, \bm{u}_k)
% \end{equation}
% The forward Euler method is based on a truncated Taylor series expansion. An error is induced at every time-step due to the truncation of the Taylor series, this is referred to as the Local Truncation Error (LTE) of the method. For the forward Euler method, the LTE is $\text{O}(dt^2)$. Hence, the method is referred to as a first order technique.

% \subsection{The Runge-Kutta Method}
% The FE method has rather poor convergence to the solution, the rate of convergence scaling linearly with $dt$. A number of efficient higher order techniques exists in the literature, among which the widely used Runge-Kutta methods are a class of methods which judiciously uses the information on the slope at more than one point to extrapolate the solution to the future time step.
% %%%%%
% The classical second order accurate Runge-Kutta method (RK2), where the LTE is $\text{O}(dt^3)$, is summarized as follows:
% \begin{equation}
%     \bm{x}_{k+1}=\bm{x}_{k} + \frac{1}{2} (\bm{k}_1 + \bm{k}_2)
% \end{equation}
% where:
% \begin{subequations}
% \begin{align*}
%     \bm{k}_1 &= dt \bm{f}(\bm{x}_k, \bm{u}_k)\\
%     \bm{k}_2 &= dt \bm{f}(\bm{x}_k + \bm{k}_1, \bm{u}_k)
% \end{align*}
% \end{subequations}
% %%%%%
% In a similar fashion Runge-Kutta methods of higher order can be developed. One of the most widely used methods for the solution of Initial Value Problems (IVPs) is the fourth order Runge-Kutta (RK4) technique, which reads as:
% \begin{equation}
%     \bm{x}_{k+1}=\bm{x}_{k} + \frac{1}{6}(\bm{k}_1+2\bm{k}_2+2\bm{k}_3+\bm{k}_4)
% \end{equation}
% with:
% \begin{subequations}
% \begin{align*}
%     \bm{k}_1 &= dt \bm{f}(\bm{x}_k, \bm{u}_k)\\
%     \bm{k}_2 &= dt \bm{f}(\bm{x}_k + \frac{\bm{k}_1}{2}, \bm{u}_k)\\
%     \bm{k}_3 &= dt \bm{f}(\bm{x}_k + \frac{\bm{k}_2}{2}, \bm{u}_k)\\
%     \bm{k}_4 &= dt \bm{f}(\bm{x}_k + \bm{k}_3, \bm{u}_k)
% \end{align*}
% \end{subequations}
% The LTE of this method is $\text{O}(dt^5)$. 

% \subsection{The Leap-Frog Method}\label{subsec:leapfrog}
% The so-called \textit{Leap-Frog} is a second order accurate method which computes $\bm{x}_{k+1}$ as:
% \begin{equation}
%     \bm{x}_{k+1}=\bm{x}_{k-1} + 2 dt \bm{f}(\bm{x}_k, \bm{u}_k)
% \end{equation}
% Any \textit{self-starting} scheme is required in order initialize the method by establishing the value of $\bm{x}$ at $k=-1$, e.g. by using Euler:
% \begin{equation}
%     \bm{x}_{-1}=\bm{x}_{0} + dt \bm{f}(\bm{x}_0, -\bm{u}_0)
% \end{equation}
% The Leap-Frog integrator is \textit{time-reversible} and this property gives it some very important advantages as it guarantees conservation of energy and angular momentum for ODEs with periodic solutions. Therefore, in situations where we are interested in long-term small changes in the properties of a nearly periodic orbit, and where even small systematic errors would mask the true solution, time-reversible integrators such as the Leap-Frog scheme are essential.
% % \subsection{\textcolor{red}{The Runge-Kutta-Fehlberg Method}}\label{subsec:RKF}

==> soa.tex <==
\section{Related Works}\label{sec:soa}

%Lists of papers
Crawling vs Stationary space robots:

Space station with robotic arm for autonomous operations

Centauro
\cite{kashiri2019centauro}
Applications:
\cite{yoshida2006capture}
Dexarm:
\cite{rusconi2008dexarm}
%Storytelling
Robotic manufacturing, assembly, and servicing utilizing in-situ resources enables the construction and maintenance of large-scale assets at significantly reduced cost. This is particularly important for space applications such as In-space assembly (ISA) \cite{mukherjee2020robotically}. Examples include large in-space assemblies like space telescopes, star-shades, commercial platforms and transportation hubs. Achieving in-situ fabrication using mobile robots is also a major goal of several terrestrial and orbital construction projects \cite{mcbryan2020comparison}. 
% can walk end-over-end, connecting to these fixtures as it travels along the exterior of the station
%Major challenges include mobility, precise manipulation, localization/mapping, and adaptability to uncertainties in the environment. The capacity to process raw materials in remote environments is also key for on-orbit, lunar, and planetary applications. In general, large ground-based facilities built in inaccessible locales could benefit greatly from in-situ robotics for inspection and servicing, and likely would necessitate a multi-robot scalable solution. 


